Serial Position Effects of Large Language Models

Large Language Models (LLMs) have shown remarkable capabilities in zero-shot learning applications, generating responses to queries using only pre-training information without the need for additional fine-tuning. This represents a significant departure from traditional machine learning approaches. Previous research has indicated that LLMs may exhibit serial position effects, such as primacy and recency biases, which are well-documented cognitive biases in human psychology. Our extensive testing across various tasks and models confirms the widespread occurrence of these effects, although their intensity varies. We also discovered that while carefully designed prompts can somewhat mitigate these biases, their effectiveness is inconsistent. These findings underscore the significance of serial position effects during the inference process, particularly in scenarios where there are no ground truth labels, highlighting the need for greater focus on addressing these effects in LLM applications.

==> Table/SerialPositionEffectsforPlain.tex <==
\begin{table*}[!hbtp]
    \setlength{\tabcolsep}{0.5mm}{}
    \begin{tabular}{l|llllllllllllllll}
          & \multicolumn{2}{l}{TACRED1} & \multicolumn{2}{l}{TACRED2} & \multicolumn{2}{l}{TACRED3} & \multicolumn{2}{l}{TACRED4} & \multicolumn{2}{l}{TACRED5} & \multicolumn{2}{l}{TACRED6} & \multicolumn{2}{l}{TACRED7} & \multicolumn{2}{l}{TACRED8} \\
Last 1    & 12           & NF           & 12           & NF           & 12           & NF           & 12           & NF           & 12           & NF           & 12           & NF           & 12           & NF           & 12           & NF           \\
Last 2    &              &              &              &              &              &              &              &              &              &              &              &              &              &              &              &              \\
Middle 1  &              &              &              &              &              &              &              &              &              &              &              &              &              &              &              &              \\
Middle 2  &              &              &              &              &              &              &              &              &              &              &              &              &              &              &              &              \\
Average 1 &              &              &              &              &              &              &              &              &              &              &              &              &              &              &              &              \\
Average 2 &              &              &              &              &              &              &              &              &              &              &              &              &              &              &              &             
\end{tabular}
    \caption{The type of \SPE{} and the the magnitude of the effects for models on various tasks.'P':Primacy Effect, 'M': Middle effect, ``R'': Recency Effect, ``N'': means no \SPE{} are detected.}
    \label{tab: serial position effects for plain}
\end{table*}
